BlessemFlood21: Advancing Flood Analysis with a High-Resolution Georeferenced Dataset for Humanitarian Aid Support

Floods are an increasingly common global threat, causing emergencies and severe damage to infrastructure. During crises, organisations such as the World Food Programme use remotely sensed imagery, typically obtained through drones, for rapid situational analysis to plan life-saving actions. Computer Vision tools are needed to support task force experts on-site in the evaluation of the imagery to improve their efficiency and to allocate resources strategically. We introduce the BlessemFlood21 dataset to stimulate research on efficient flood detection tools. The imagery was acquired during the 2021 Erftstadt-Blessem flooding event and consists of high-resolution and georeferenced RGB-NIR images. In the resulting RGB dataset, the images are supplemented with detailed water masks, obtained via a semi-supervised human-in-the-loop technique, where in particular the NIR information is leveraged to classify pixels as either water or non-water. We evaluate our dataset by training and testing established Deep Learning models for semantic segmentation. With BlessemFlood21 we provide labeled high-resolution RGB data and a baseline for further development of algorithmic solutions tailored to flood detection in RGB imagery.

==> tmp.tex <==
% \subsection{Dataset Quality.}
% \paragraphc{Dataset Quality Assessment.}
% % Three represantative sample
% The accuracy of the ground truth generated for binary semantic segmentation in post-flood imagery is evaluated using visual qualitative assessment, as there are no specific quantitative metrics available. The ground truth was established employing a framework involving human in the loop. In Figure \ref{fig:Generate Ground Truth Samples}, we present three representative sample tiles to illustrate the resulting mask quality.
% % Rural
% In Figure \ref{fig:Generate Ground Truth Samples}a, the landscape is reshaped by flooding consequences. Rural Damage. The first image presents consequences of flooding, reshaping the landscape. It depicts a crop field now visibly affected by the aftermath of flooding. The image captures flooded trees and the newly formed edge resulting from a triggered landslide.
% % Urban
% In Figure \ref{fig:Generate Ground Truth Samples}b, attention is drawn to the edge of an urban environment in the town of Erftstadt, specifically near a gravel pit. The landscape shows evidence of numerous floodwater residuals. Partially flooded buildings serve as reminders of the event's destructive nature. Additionally, scattered debris emphasizes the extent of damage and the recovery process's challenges.
% % River
% Finally, in Figure \ref{fig:Generate Ground Truth Samples}c a river scene with a bridge and residual flood water is shown. It demonstrates the complexity of assessing damage in a dynamic river environment. The presence of shadows creates additional challenges, adding complexity to the analysis. The turbidity of flowing river water is also noteworthy, emphasizing the difficulty of accurately assessing the full extent of the impact. 
% % Short summary of the quality achieved
% Our human in the loop framework demonstrates resilience in tackling demanding environmental factors, as shown by its performance in the river example shown in Figure~\ref{fig:Generate Ground Truth Samples}c. Of particular note is its ability to effectively handle scenarios involving shadows, demonstrating a good level for the case of inhomogeneous lighting conditions.  Moreover, the framework is exemplary in delineating complex boundaries in the aftermath of a flood, as demonstrated in Figure~\ref{fig:Generate Ground Truth Samples}a. The framework's ability to precisely define complex boundaries is fundamental to its usefulness in characterising flood-induced damages accurately. This contributes to the reliability of the framework as a tool for image segmentation in environmental analysis. 
% % Note class imbalance
% It is important to note that the resulting dataset exhibits a notable bias towards the non-water class, with about 85\% of pixels belonging to this category. This bias is primarily attributed to the prevalence of river scenes in the dataset, wherein the accurate depiction of rivers experiencing elevated water levels contributes valuable flood analysis data at a high spatial resolution. 
% % Final summary
% The ground truth dataset generated exhibits exceptional accuracy in delineating water masks, providing a comprehensive portrayal of complex flooded landscapes. This dataset provides detailed insights into spatially resolved flood scenarios, with a particular focus on the challenges inherent in river inundation near urban cities. Its precision allows for a better understanding of flood dynamics, thereby contributing to the development of mitigation strategies.
% %
% \begin{figure}[h!]
%   \centering
% {\begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_1_img.JPG}
%   \end{subfigure}%
%   \hspace{3 mm}
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_1_mask.JPG}
%   \end{subfigure}%
%   \subcaption{Rural damage on crop field.}
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_2_img.JPG}
%   \end{subfigure}%
%   \hspace{3 mm}
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_2_mask.JPG}
%   \end{subfigure}%
%   \subcaption{Urban damage with flooded infrastructure and debris.}
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_5_img.JPG}
%   \end{subfigure}%
%   \hspace{3 mm}
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_5_mask.JPG}
%   \end{subfigure}%
% \subcaption{River Sample with turbid water and floodwater residuals.}
% }
% \caption{Three sample pair tiles of preprocessed imagery and generated ground truth on the edges of the gravel pit, Erftstadt}
% \label{fig:Generate Ground Truth Samples}
% \end{figure}
% %

% Model suitability
% Model overcome shadows and show good performance on boundaries as well as on muddy water as well as turibid water


% \paragraphc{Model Performance.}
% % Model suitability
% % Model overcome shadows and show good performance on boundaries as well as on muddy water as well as turbid water
% % QUalitative
% Figure \ref{fig:Intermodel Comparison} shows successful segmentation by all three models despite the significant class imbalance present in the imagery. The predictions are similar and successfully detect larger details and smooth boundary delineation, as well as turbid and muddy water.  However, the models consistently demonstrate a performance limitation and fail to capture finer details represented by smaller soil residuals. Smaller objects, which are visible within regions enclosed by muddy water in the center of the predicted masks, are often either undetected or incorrectly classified as water.


% \begin{figure*}[t]
%   \centering
%   % Subfigure 1: Original
%   \begin{subfigure}{0.18\linewidth}
%     \includegraphics[width=\linewidth]{img/test_set_orig.jpg}
%     \caption{Original}
%     \label{fig:subfig1}
%   \end{subfigure}
%   \hfill
%   % Subfigure 2: Ground Truth
%   \begin{subfigure}{0.18\linewidth}
%     \includegraphics[width=\linewidth]{img/test_set_gt.jpg}
%     \caption{Ground Truth}
%     \label{fig:subfig2}
%   \end{subfigure}
%   \hfill
%   % Subfigure 3: UNet++ Predicted Mask
%   \begin{subfigure}{0.18\linewidth}
%     \includegraphics[width=\linewidth]{img/test_set_upp12.jpg}
%     \caption{UNet++}
%     \label{fig:subfig3}
%   \end{subfigure}
%   \hfill
%   % Subfigure 4: DeepLabV3+ Prediction
%   \begin{subfigure}{0.18\linewidth}
%     \includegraphics[width=\linewidth]{img/test_set_dl3p12.JPG}
%     \caption{DeepLabV3+}
%     \label{fig:subfig4}
%   \end{subfigure}
%   \hfill
%   % Subfigure 5: LinkNet3 Prediction
%   \begin{subfigure}{0.18\linewidth}
%     \includegraphics[width=\linewidth]{img/test_set_sf12.JPG}
%     \caption{SegFormer}
%     \label{fig:subfig5}
%   \end{subfigure}

%   \caption{Qualitative comparison of ground truth and predictions obtained after finetuning with 100 epochs.}
%   \label{fig:Intermodel Comparison}
% \end{figure*}



% % \begin{table*}[h!]
% % \centering
% % \begin{tabular}{lcccc}
% % \toprule
% % Model & Encoder & Params & IoU (\%) & Dice (\%) \\
% % \midrule
% % DeepLabV3+  & Resnet-50 & 26.7 M &  90.6 & 95.1 \\ 
% % UNet++      & Resnet-50 & 49.0 M &  84.2 & 91.4 \\ 
% % SegFormer-b5& Hierarchical ViT & 84.6 M &  75.4 & 78.4 \\ 
% % \bottomrule
% % \end{tabular}
% % \caption{Performance Comparison of Models on the Test Set of BlessemFlood21.}
% % \label{tab:model_comparison_blessem}
% % \end{table*}

% \begin{table}[h!]
% \centering
% \begin{tabular}{p{1.8cm}p{2.cm}p{1.cm}p{0.8cm}p{0.8cm}}
% \toprule
% Model & Encoder & Params & IoU (\%) & Dice (\%) \\
% \midrule
% DeepLabV3+  & Resnet-50 & 26.7 M &  90.6 & 95.1 \\ 
% UNet++      & Resnet-50 & 49.0 M &  84.2 & 91.4 \\ 
% SegFormer-b5& Hierarchical ViT & 84.6 M &  75.4 & 78.4 \\ 
% \bottomrule
% \end{tabular}
% \caption{Performance Comparison of Models on the Test Set of BlessemFlood21.}
% \label{tab:model_comparison_blessem}
% \end{table}



% % Quantitative 
% For quantitative evaluation, we use Intersection over Union (IoU) and Dice Score metrics (Dice). Table~\ref{tab:model_comparison_blessem} shows the model performance of DeepLabV3+, UNet++, and SegFormer for the test set.
% % 
% % All models perform well on the dataset
% Both IoU and Dice values indicate strong performance across all models achieving more than 75\% IoU and 78\% on the test set despite the high class imbalance. This is consistent with the visual observations shown in Figure \ref{fig:Intermodel Comparison}.
% %
% % Final Remarks:
% In summary, our baseline demonstrates good performance in water segmentation within the Blessem21Flood dataset. The qualitative analysis indicates successful detection of larger details, although there are limitations in segmenting smaller objects. Quantitative performance metrics further confirm the overall good results of the applied models. This indicates the suitability of our dataset for semantic segmentation tasks.


% \paragraphc{Contribution Importance.}
% % inter-dataset benchmark
% % COmparison to existing datasets
% The importance of BlessemFlood21 is further emphasised by our investigation into the uniqueness of the information obtained by models, highlighting the distinctive features of our dataset. To support this, we evaluated the insufficiency of replacing the acquired knowledge with alternative datasets. We choose FloodNet because of its similar acquisition setup to our dataset. The performance of our models trained on BlessemFlood21 is evaluated on the test set of FloodNet. Next, we retrained these models for 100 epochs using FloodNet and tested their performance on BlessemFlood21. 
% %
% % Results
% The results show a consistent decline in model performance for both scenarios, as measured by Intersection over Union (IoU) and Dice Score (Dice). Despite extensive retraining on FloodNet, the models still exhibited poor performance when applied to BlessemFlood21. Models trained on FloodNet achieved the highest overall IoU of only 10.5\% and a Dice Score of 19.0\%. Based on these results, we emphasize the unique features of our image and its significant contribution to further research.
%

% This study presents the BlessemFlood21 dataset, created using an iterative high-precision human in the loop annotation framework. Firstly, we demonstrate that incorporating NIR information enhances water highlighting and improves the quality of generated water masks. Secondly, we apply well-established state-of-the-art models for segmentation as a baseline on our dataset, achieving excellent performance with an IoU of 90.6\% and a Dice Score of 95.1\%. Regarding the excellent scores in both metrics, we confirm that BlessemFlood21 is helpful for water segmentation using DL models and its quality is good. Additionally, we conclude that the quality is good. Lastly, we highlight the uniqueness of the features contained in our dataset as well as its necessity. FloodNet models were used to test their performance on BlessemFlood21. The limitations observed in performance highlight the complexity of domain adaptation, where transferring knowledge across datasets with varying features is non-trivial. This result emphasizes the need for domain-specific datasets, such as BlessemFlood21, and supports the argument that current datasets are inadequate in capturing the distinct and diverse features of particular domains. Therefore, specialised datasets are required to enhance model generalisation and performance.


% \section{Formatting your paper}
% \label{sec:format}

% All printed material, including text, illustrations, and charts, must be kept
% within a print area of 7 inches (178 mm) wide by 9 inches (229 mm) high. Do
% not write or print anything outside the print area. The top margin must be 1
% inch (25 mm), except for the title page, and the left margin must be 0.75 inch
% (19 mm).  All {\it text} must be in a two-column format. Columns are to be 3.39
% inches (86 mm) wide, with a 0.24 inch (6 mm) space between them. Text must be
% fully justified.



% \section{PAGE TITLE SECTION}
% \label{sec:pagestyle}

% The paper title (on the first page) should begin 1.38 inches (35 mm) from the
% top edge of the page, centered, completely capitalized, and in Times 14-point,
% boldface type.  The authors' name(s) and affiliation(s) appear below the title
% in capital and lower case letters.  Papers with multiple authors and
% affiliations may require two or more lines for this information.

% \section{TYPE-STYLE AND FONTS}
% \label{sec:typestyle}

% To achieve the best rendering in the proceedings, we
% strongly encourage you to use Times-Roman font.  In addition, this will give
% the proceedings a more uniform look.  Use a font that is no smaller than ten
% point type throughout the paper, including figure captions.

% In ten point type font, capital letters are 2 mm high.  If you use the
% smallest point size, there should be no more than 3.2 lines/cm (8 lines/inch)
% vertically.  This is a minimum spacing; 2.75 lines/cm (7 lines/inch) will make
% the paper much more readable.  Larger type sizes require correspondingly larger
% vertical spacing.  Please do not double-space your paper.  True-Type 1 fonts
% are preferred.

% The first paragraph in each section should not be indented, but all the
% following paragraphs within the section should be indented as these paragraphs
% demonstrate.

% \section{MAJOR HEADINGS}
% \label{sec:majhead}

% Major headings, for example, "1. Introduction", should appear in all capital
% letters, bold face if possible, centered in the column, with one blank line
% before, and one blank line after. Use a period (``.") after the heading number,
% not a colon.

% \subsection{Subheadings}
% \label{ssec:subhead}

% Subheadings should appear in lower case (initial word capitalized) in
% boldface.  They should start at the left margin on a separate line.
 
% \subsubsection{Sub-subheadings}
% \label{sssec:subsubhead}

% Sub-subheadings, as in this paragraph, are discouraged. However, if you
% must use them, they should appear in lower case (initial word
% capitalized) and start at the left margin on a separate line, with paragraph
% text beginning on the following line.  They should be in italics.

% \section{PRINTING YOUR PAPER}
% \label{sec:print}

% Print your properly formatted text on high-quality, 8.5 x 11-inch white printer
% paper. A4 paper is also acceptable, but please leave the extra 0.5 inch (12 mm)
% empty at the BOTTOM of the page and follow the top and left margins as
% specified.  If the last page of your paper is only partially filled, arrange
% the columns so that they are evenly balanced if possible, rather than having
% one long column.

% In LaTeX, to start a new column (but not a new page) and help balance the
% last-page column lengths, you can use the command ``$\backslash$pagebreak'' as
% demonstrated on this page (see the LaTeX source below).

% \section{PAGE NUMBERING}
% \label{sec:page}

% Please do {\bf not} paginate your paper.  Page numbers, session numbers, and
% conference identification will be inserted when the paper is included in the
% proceedings.

% \section{ILLUSTRATIONS, GRAPHS, AND PHOTOGRAPHS}
% \label{sec:illust}

% Illustrations must appear within the designated margins.  They may span the two
% columns.  If possible, position illustrations at the top of columns, rather
% than in the middle or at the bottom.  Caption and number every illustration.
% All illustrations should be clear wwhen printed on a black-only printer. Color
% may be used.

% Since there are many ways, often incompatible, of including images (e.g., with
% experimental results) in a LaTeX document, below is an example of how to do
% this \cite{Lamp86}.

% Below is an example of how to insert images. Delete the ``\vspace'' line,
% uncomment the preceding line ``\centerline...'' and replace ``imageX.ps''
% with a suitable PostScript file name.
% -------------------------------------------------------------------------
% \begin{figure}[htb]

% \begin{minipage}[b]{1.0\linewidth}
%   \centering
% % \centerline{\epsfig{figure=image1.ps,width=8.5cm}}
%   \vspace{2.0cm}
%   \centerline{(a) Result 1}\medskip
% \end{minipage}
% %
% \begin{minipage}[b]{.48\linewidth}
%   \centering
% % \centerline{\epsfig{figure=image3.ps,width=4.0cm}}
%   \vspace{1.5cm}
%   \centerline{(b) Results 3}\medskip
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.48\linewidth}
%   \centering
% % \centerline{\epsfig{figure=image4.ps,width=4.0cm}}
%   \vspace{1.5cm}
%   \centerline{(c) Result 4}\medskip
% \end{minipage}
% %
% \caption{Example of placing a figure with experimental results.}
% \label{fig:res}
% %
% \end{figure}

% To start a new column (but not a new page) and help balance the last-page
% column length use \vfill\pagebreak.
% -------------------------------------------------------------------------
% \vfill
% \pagebreak


% \section{FOOTNOTES}
% \label{sec:foot}

% Use footnotes sparingly (or not at all!) and place them at the bottom of the
% column on the page on which they are referenced. Use Times 9-point type,
% single-spaced. To help your readers, avoid using footnotes altogether and
% include necessary peripheral observations in the text (within parentheses, if
% you prefer, as in this sentence).


% \section{COPYRIGHT FORMS}
% \label{sec:copyright}

% You must also electronically sign the IEEE copyright transfer
% form when you submit your paper. We {\bf must} have this form
% before your paper can be sent to the reviewers or published in
% the proceedings. The copyright form is provided through the IEEE
% website for electronic signature. A link is provided upon
% submission of the manuscript to enter the IEEE Electronic
% Copyright Form system.

% \section{REFERENCES}
% \label{sec:ref}

% List and number all bibliographical references at the end of the paper.  The references can be numbered in alphabetic order or in order of appearance in the document.  When referring to them in the text, type the corresponding reference number in square brackets as shown at the end of this sentence~\cite{C2}.

% References should be produced using the bibtex program from suitable
% BiBTeX files (here: strings, refs, manuals). The IEEEbib.bst bibliography
% style file from IEEE produces unsorted bibliography list.


% \section{Annotation Framework}

% % Introduction
% When annotating, the primary goal is to generate a georeferenced mask for semantic segmentation, which classifies each pixel in its respective mosaic as either water or non-water. 
% %
% % Motivate Annotations
% With a vast amount of pixels and a lack of ground truth, automating the labelling process becomes imperative. 
% %
% % Motivate ML
% Labeling raw image material is a challenging task due to unpredictable lighting conditions, obstacles, debris, and diverse landscapes. In addition, flooded regions exhibit subtle visual patterns that require careful consideration. In view of the intricate nature of the imagery and the objective to hasten manual analysis, machine learning is applied.
% %
% % Human in the loop
% To tackle these challenges, we implement a human in the loop framework comprising preprocessing, human annotators, segmentation using machine learning, and subsequent visual assessment.
% %
% % Framework Architecture
% % Labeling guidelines
% During annotation process, we define the classification criteria. We identify pixels corresponding to natural water bodies, flooded areas, and lakes, along with their residual areas categorised as water. Conversely, objects like buildings, roads, vehicles and mud are classified as non-water.
% %
% % Preprocessing Steps
% The RGB-NIR orthomosaic is divided into 4623 tiles of 512 x 512 pixels each to overcome hardware limitations. To address the issue of low contrast in the raw imagery, a pixel value stretching technique is applied to individual tiles. This involves normalising the values of each tile within the range defined by the 2nd and 90th percentiles of the entire mosaic. This process produces consistently normalised images with enhanced contrast. The subsequent step is to transform the four-channel RGB-NIR tiles into false-color RGB representations by remapping. This technique involves combining the existing channels into a single three-channel image, resulting in a false-colour RGB composition. 
% Drawing on expertise from Remote Sensing, where water has been shown to absorb light in the NIR spectrum \cite{ahn20estimatingwaterabsorbsnir}, the representation integrates the NIR band. This feature is particularly useful for highlighting areas with water abundance, and improving mask generation accuracy. After systematically evaluating different band configurations, we identify the combination of Near-Infrared (NIR), Blue (B), and Red (R) channels as the most beneficial. 

% % Annotation
% After preprocessing the images, we use Ilastik \cite{berg19ilastik} for the annotation and segmentation process. Ilastik is a free and open source toolkit for image analysis tasks, including semantic segmentation. It applies interactive supervised machine learning, where pixel classification is guided by sparse labels. This feature enables faster and higher quality results compared to time-consuming and error-prone manual pixel-wise image annotation. A subset of tiles is labelled using sparse brush strokes. During  annotation of water, the emphasis is placed on labelling the boundaries of flooded areas or rivers in particular as they represent the highest uncertainty during segmentation.


% % Random Forest resulting segmentation
% In Ilastik, we select a Random Forest \cite{breiman01randomforest} classifier for segmentation, using its pixel classification pipeline. We apply the classifier, which consists of 100 trees, to the coarsely annotated tiles. 

% % Evaluation
% The lack of precise ground truth data regarding land cover types depicted in our imagery poses a notable challenge in our assessment approach for flooded landscapes. Subsequently, evaluating it based on metrics is not a viable option. In order to counteract this drawback during the evaluation phase, we rely on comparing the tiles' false colour and true colour representations visually. This methodology allows us to derive accurate conclusions despite the absence of ground truth data. With such an approach we reduce the residual uncertainty that may endure because of illumination effects, such as cloud shadows and pixel value similarity between mud and muddy water.

% % Iterative correction
% Initial segmentation masks achieve high precision by delivering mostly accurate shapes. However, some label noise is still present. Thus, a refinement process involving human interaction is chosen to ensure masks of the highest quality.  We examine the imagery and, in the event of a rejection, introduce additional labels into the model, initiating a process of retraining. This iterative cycle continues until the resulting mask detail achieves the desired accuracy standards. 


% % Geoinfo was transferred
% After generating the ground truth masks, georeferences are transferred from their raw tile counterpart.
% % Provision of two mosaics only
% Finally, we create two mosaics that represent the dataset. One for the imagery acquired by drone and one that represents the water mask. In response to real-world humanitarian aid scenarios, we exclude non-RGB information, aligning with practical limitations.



fließtext contribution

xBd and others shorten


annotation framework 

manual annotation takes too long and error-prone
Semi automated with human in the loop
classical machine learning based on Random Forest is employed


using NIR is absorbs in water

nach machine learning


During annotation the following criteria are set: 


%
% Single address.
% ---------------
%\name{Author(s) Name(s)\thanks{Thanks to XYZ agency for funding.}}
%\address{Author Affiliation(s)}
%
% For example:
% ------------
%\address{School\\
%	Department\\
%	Address}
%
% Two addresses (uncomment and modify for two-address case).
% ----------------------------------------------------------
%\twoauthors
%  {A. Author-one, B. Author-two\sthanks{Thanks to XYZ agency for funding.}}
%	{School A-B\\
%	Department A-B\\
%	Address A-B}
%  {C. Author-three, D. Author-four\sthanks{The fourth author performed the work
%	while at ...}}
%	{School C-D\\
%	Department C-D\\
%	Address C-D}
%
% More addresses (uncomment and modify for more address case)
% Consider using \fourauthors, \fiveauthors, etc. 
% You shoulb be able to grop authors based on Schools, as before.

% \threeauthors
%   {Vladyslav Polushko $^{1, 2}$ \\ Andreas Weinmann$^{2 }$ \\ Thomas März$^{2}$}
%   {$^{2}$Darmstadt University of Applied Sciences\\	Mathenmatics and Science \\	Address B}
%   {Alexander Jenal$^{\,3}$ \\ Jens Bongartz$^{3}$\\ Immanuel Weber$^{3}$}
%   {$^{3}$Koblenz University of Applied Sciences\\Debartment B \\	Address B}
%   {Damjan Hatic$^{1}$ \\ Markus Rauhut$^{1}$ \\ Ronald Rösch$^{1}$}
%   {$^{1}$Fraunhofer Institute for Industrial Mathematics ITWM \\	Image Processing \\	Address A}


% \oneauthor
%   {Vladyslav Polushko $^{1, 2}$ \\ Andreas Weinmann$^{2 }$ \\ Thomas März$^{2}$}
%   {$^{2}$Darmstadt University of Applied Sciences\\	Mathenmatics and Science \\	Address B}
%   {Alexander Jenal$^{\,3}$ \\ Jens Bongartz$^{3}$\\ Immanuel Weber$^{3}$}
%   {$^{3}$Koblenz University \\Debartment B \\	Address B}
%   {Damjan Hatic$^{1}$ \\ Markus Rauhut$^{1}$ \\ Ronald Rösch$^{1}$}
%   {$^{1}$Fraunhofer Institute for Industrial Mathematics ITWM \\	Image Processing \\	Address A} 

% \name{Vladyslav Polushko \textsuperscript{1, 2}
% \and Alexander Jenal \textsuperscript{3}
% \and Jens Bongartz \textsuperscript{3}
% \and Immanuel Weber\textsuperscript{3}
% \and Damjan Hatic \textsuperscript{1}
% \and Ronald Rösch \textsuperscript{1}
% \and Thomas März \textsuperscript{2}
% \and Markus Rauhut \textsuperscript{1}
% \and Andreas Weinmann \textsuperscript{2}    
% }
% \address{\textsuperscript{1}Fraunhofer Institute for Industrial Mathematics ITWM\\ 
% \textsuperscript{2}Darmstadt University of Applied Sciences 
% \\ \textsuperscript{3}Koblenz University of Applied Sciences}


% \begin{figure}[h!]
%   \centering
% {\begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_1_img.JPG}
%   \end{subfigure}%
%   \hspace{3 mm}
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_1_mask.JPG}
%   \end{subfigure}%
%   \subcaption{Rural damage on crop field.}
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_2_img.JPG}
%   \end{subfigure}%
%   \hspace{3 mm}
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_2_mask.JPG}
%   \end{subfigure}%
%   \subcaption{Urban damage with flooded infrastructure and debris.}
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_5_img.JPG}
%   \end{subfigure}%
%   \hspace{3 mm}
%   \begin{subfigure}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/sample_5_mask.JPG}
%   \end{subfigure}%
% \subcaption{River with turbid water and floodwater residuals.}
% }
% \caption{Three representative sample pairs of preprocessed imagery (left) and generated ground truth water masks (right). White pixels in the masks indicate water pixels.}
% \label{fig:Generate Ground Truth Samples}
% \end{figure}
% %



%  \item \textbf{Contribution 2:} Application of established Deep Learning models, providing a valuable baseline for further flood analysis. 
%\end{itemize}


%
%
% Contributions
% In response to the increasing frequency and severity of global floods attributed to climate change, this work makes two significant contributions to support rapid and effective humanitarian flood analysis. Firstly, we use exclusively imagery acquired by gyrocopters to create the novel BlessemFlood21 dataset.

% , making it the first of its kind for European flooding events. %This addresses the scarcity of flood datasets appropriate for semantic segmentation. 
%
% Additionally, we use deep learning models to perform semantic segmentation on this dataset, taking a ground-breaking approach. This study offers significant insights into the use of these models in a challenging environment. By testing the applicability of the dataset with state-of-the-art segmentation models, it sets a foundation for future research and the creation of deep learning algorithms customised to support humanitarian groups in flood response and rescue.

%In summary, our contributions as follow:
%\begin{itemize}
%  \item \textbf{Contribution 1:} Development of the BlessemFlood21 dataset, featuring high spatial resolution and tailored for semantic segmentation of water.   
%  \item \textbf{Contribution 2:} Application of established Deep Learning models, providing a valuable baseline for further flood analysis. 
%\end{itemize}

% The dataset boasts an impressive spatial resolution of 15 cm and nadir acquisition.
1- 4 refernzen
6 malawi suchen
